Differentiable Window for Dynamic Local Attention

We propose Differentiable Window, a new neural module and general purpose component for dynamic window selection. While universally applicable, we demonstrate a compelling use case of utilizing Differentiable Window to improve standard attention modules by enabling more focused attentions over the input regions. We propose two variants of Differentiable Window, and integrate them within the Transformer architecture in two novel ways. We evaluate our proposed approach on a myriad of NLP tasks, including machine translation, sentiment analysis, subject-verb agreement and language modeling. Our experimental results demonstrate consistent and sizable improvements across all tasks.

==> archive.tex <==
\vspace{-0.3em}
\subsection{Sentiment Analysis}\label{subsec:result:sentiment_analysis}

We evaluate our models on the Stanford Sentiment Treebank (SST) \cite{D13-1170} and IMDB sentiment analysis tasks. We compare our attention methods (incorporated into the Transformer encoder) with the encoders of Vaswani et al. (  \citeyear{vaswani2017attention}), Shaw et al.  (\citeyear{Shaw18-relative}) and Yang et al. (\citeyear{yang-etal-2018-modeling}). 

%We report accuracy numbers.

%original Transformer  and Transformer with relative position .
%Model evaluations are measured by binary classification accuracy. 

\vspace{-1em}
\paragraph{Training Setup.} As the datasets for sentiment analysis tasks are quite small compared to the MT datasets, we used \textit{tiny versions} of our models as well as the baselines.\footnote{As specified in https://github.com/tensorflow/tensor2tensor.} Specifically, the models consist of a 2-layer Transformer \textbf{encoder} with 4 attention heads, 128 hidden dimensions and 512 feedforward inner dimensions. In these experiments, our attention methods are applied only to the first layer of the network. We trained for 3,000 and 10,000 updates for SST and IMDB tasks, respectively on a single GPU machine.

%We only used 1 GPU without gradient aggregation. 

%involve comparably small datasets, 
 
 \begin{table}[t]
\begin{center}
\resizebox{0.75\columnwidth}{!}{%
%\setlength\tabcolsep{1.2pt}
\begin{tabular}{lcc} 
\toprule
% {\bf Tasks}                 &Sentiment &Subject Verb Agreement\\
{\bf Model}                  & {\bf STT} & {\bf IMDB} \\
\midrule
Vaswani et al. (  \citeyear{vaswani2017attention})           & 79.36 & 83.65      \\
Shaw et al.  (\citeyear{Shaw18-relative})  & 79.73 & 84.61  \\
Yang et al. (\citeyear{yang-etal-2018-modeling}) & 79.24 & 84.13 \\
\midrule
% Soft Local Encoder            & 79.24 & 84.13         \\
Enc (MW)            & 79.70 & 85.09  \\
% Global Local Encoder            & 81.77 & 86.53        \\
Enc (AW)        & \textbf{82.13}    & \textbf{87.98}   \\

\bottomrule
\end{tabular}
%\setlength\tabcolsep{6pt}
}
\vspace{-0.3em}
\caption{Sentiment analysis accuracy on Stanford Sentiment Treebank (SST) and IMDB datasets.}
\label{table:sentiment}
\end{center}
\vspace{-1em}
\end{table}
 
\vspace{-1em}
\paragraph{Results.} 
Table \ref{table:sentiment} shows the results. Our multiplicative window approach ({Enc (MW)}) achieves up to 79.7\% and 85.1\% accuracy in SST and IMDB, exceeding Transformer   \cite{vaswani2017attention} by 0.4\% and 1.35\%, respectively. Our additive window attention ({Enc (AW)}) renders even more improvements. Specifically, it outperforms Transformer with relative position (Shaw et al. \citeyear{Shaw18-relative}) by 2.4\% and 3.37\%, reaching 82.13\% and 87.98\% accuracy in SST and IMDB, respectively. In fact, the results demonstrate consistent trends with our earlier MT experiments. That is, additive window attention outdoes its multiplicative counterpart in the encoder, where the entire key sequence is available. %and global context can be extracted.


\vspace{-0.2em}
\subsection{Subject Verb Agreement}\label{subsec:result:sva}
Subject Verb Agreement or SVA \cite{TACL972} is the task to classify whether the subject and the verb in a sentence agree in number (both are plural or singular). For example, the sentence `My \textbf{dog} always \textbf{growls} at the postal carrier' is a \textit{positive} example. We followed the data splitting settings from tensor2tensor gihub. We used the same training setup as in sentiment analysis, except that we trained the models (our models and the baselines) for 10,000 updates. 

%We also compare our approaches with Transformer \cite{vaswani2017attention} and Transformer with relative position \cite{Shaw18-relative}. 


\begin{table}[t]
\begin{center}
\resizebox{0.60\columnwidth}{!}{%
%\setlength\tabcolsep{1.2pt}
\begin{tabular}{lc} 
\toprule
{\bf Model}                  & {\bf Acc}  \\
\midrule
Vaswani et al. (  \citeyear{vaswani2017attention})           & 94.48       \\
Shaw et al.  (\citeyear{Shaw18-relative})  & 95.27 \\
Yang et al. (\citeyear{yang-etal-2018-modeling}) & 95.00 \\
\midrule
% Soft Local Encoder            & 96.62         \\
Enc (MW)           & 95.95         \\
% Global Local Encoder            & 95.55       \\
Enc (AW)            & \textbf{96.19}         \\
\bottomrule
\end{tabular}
%\setlength\tabcolsep{6pt}
}
\vspace{-0.3em}
\caption{Results on Subject Verb Agreement Task.}
\label{table:SVA}
\end{center}
\vspace{-1em}
\end{table}


\vspace{-1em}
\paragraph{Results.}
Table \ref{table:SVA} presents the results of our SVA experiments, which exhibit similar patterns as other tasks. Particularly, our Transformer encoders applying multiplicative ({Enc (AW)}) and additive ({Enc (MW)}) window attentions achieve 96.19\% and 95.95\% accuracy respectively, which are 0.92\% and 0.6\% improvements over  Shaw et al. (\citeyear{Shaw18-relative}).


% base, epoch 1: Loss: 3.9098, Perplexity: 49.89
\vspace{-0.2em}

\subsection{Language Modeling}\label{subsec:result:lm}

Finally, to demonstrate our proposed methods as effective general purpose NLP components, we evaluate them on the 1 Billion Word LM Benchmark dataset \cite{Chelba-LM}.
The dataset contains 768 million words of data compiled from WMT 2011 News Crawl data, with a vocabulary of 32,000 words. We used its held-out data as the test set.
%Performances are measured by \textit{perplexity} score. %As previously, we compare our dynamic window-based methods with Transformer \cite{vaswani2017attention} and Transformer with relative position \cite{Shaw18-relative}.

\vspace{-1em}
\paragraph{Training Setup.} As the LM dataset is considerably large, we used the same model settings as adopted in our MT experiments.  For these experiments, we only trained the models on virtually 4 GPUs for 100,000 \textit{updates} using gradient aggregation on a single GPU machine. 
% The effective batch size is 16,384 tokens. 
Note that only the self-attention based autoregressive \textbf{decoder} of the Transformer framework is used in this task. Therefore, the method of Yang et al. (\citeyear{yang-etal-2018-modeling}) is not applicable to this task.

\begin{table}[t]
\begin{center}
\resizebox{0.65\columnwidth}{!}{%
%\setlength\tabcolsep{1.2pt}
\begin{tabular}{lc} 
\toprule
{\bf Model}                  & {\bf Perplexity}  \\
\midrule
Vaswani et al. (  \citeyear{vaswani2017attention})  & 46.37       \\
Shaw et al.  (\citeyear{Shaw18-relative})       & 46.13\\
\midrule
% Soft Local Encoder            & 96.62         \\
% Full De(AW)     & 45.26      \\
Dec (MW)            & \textbf{44.00}         \\
Dec (AW)            & 44.95         \\
% Full De(MW)       & 44.92       \\

% Global Local Encoder            & 95.55       \\
\bottomrule
\end{tabular}
%\setlength\tabcolsep{6pt}
}
\vspace{-0.3em}
\caption{Perplexity scores on 1-billion-word language modeling benchmark (the lower the better).}
\label{table:lm}
\end{center}
\vspace{-1.8em}
\end{table}


\vspace{-1em}
\paragraph{Results.} 
Table \ref{table:lm} shows the \textbf{perplexity} scores. As can be seen, our multiplicative and additive window attention models both surpass Transformer \cite{vaswani2017attention} by 2.37 and 1.42 points respectively, reaching 44.00 and 44.95 perplexity scores respectively.
% They also outperform Transformer with relative position \cite{Shaw18-relative} by 2.13 and 1.18 points.
In addition, it is noteworthy that similar to MT experiments, multiplicative attention  outperforms the additive one on this task, where the decoder is used. 
% This observation in the LM task is consistent with MT experiments as well as the ablation study in MT. 
This further reinforces the claim that where the global context is not \textit{fully} available like in the decoder, the incomplete global context may induce noises into the model. Thus, it is effective to embrace dynamic local window attention to suppress the global context, for which the  multiplicative window attention is designed.

% \alert{Some task-specific challenges can be introduced.. }
